Unique Information via Dependency Constraints

The partial information decomposition (PID) is perhaps the leading proposal for resolving information shared between a set of sources and a target into redundant, synergistic, and unique constituents. Unfortunately, the PID framework has been hindered by a lack of a generally agreed-upon, multivariate method of quantifying the constituents. Here, we take a step toward rectifying this by developing a decomposition based on a new method that quantifies unique information. We first develop a broadly applicable method---the dependency decomposition---that delineates how statistical dependencies influence the structure of a joint distribution. The dependency decomposition then allows us to define a measure of the information about a target that can be uniquely attributed to a particular source as the least amount which the source-target statistical dependency can influence the information shared between the sources and the target. The result is the first measure that satisfies the core axioms of the PID framework while not satisfying the Blackwell relation, which depends on a particular interpretation of how the variables are related. This makes a key step forward to a practical PID.

==> cmechabbrev.tex <==
% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}\xspace}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}\xspace}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}\xspace}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}\xspace}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}\xspace}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}\xspace}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}\xspace}
\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}\xspace}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}      {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\BiInfinity}        { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}        { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past}      { \smash{\overleftarrow {\MeasSymbol}} }
\newcommand{\past}      { \smash{\overleftarrow {\meassymbol}} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}    { \smash{\overrightarrow{\MeasSymbol}} }
\newcommand{\future}    { \smash{\overrightarrow{\meassymbol}} }
\newcommand{\futureprime}       { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}       { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}      { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL}     { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL}     { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}        { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}      { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}        { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }

% Causal states and epsilon-machines
\newcommand{\CausalState}       { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}       { \sigma }
\newcommand{\CausalStateSet}    { \boldsymbol{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}       { {\cal R}^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}       { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \boldsymbol{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \boldsymbol{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}      { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}      { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}             { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}               {C_\mu}
\newcommand{\hmu}               {h_\mu}
\newcommand{\EE}                {{\bf E}}
\newcommand{\TI}                {{\bf T}}
\newcommand{\SyncI}        {{\bf S}}
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}                {\chi}

% Causal Irreversibility
\newcommand{\CI}                {\Xi}
\newcommand{\ReverseMap}        {r}
\newcommand{\ForwardMap}        {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\boldsymbol{\EstCausalState}}
\newcommand{\EstCausalFunc}     {\widehat{\epsilon}}
\newcommand{\EstCmu}            {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}        { \mathcal{A}}
\newcommand{\insymbol}          { a}
\newcommand{\OutAlphabet}       { \mathcal{B}}
\newcommand{\outsymbol}         { b}
\newcommand{\InputSimple}       { X}
\newcommand{\inputsimple}       { x}
\newcommand{\BottleneckVar}     {\tilde{\InputSimple}}
\newcommand{\bottleneckvar}     {\tilde{\inputsimple}}
\newcommand{\InputSpace}        { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}       { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}       { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}        { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}      { Y}
\newcommand{\outputsimple}      { y}
\newcommand{\OutputSpace}       { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}        { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}        { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}      { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}      { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne}     { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone}     { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}        {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}        {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}       {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}        {{\InputPast}^{L}}
\newcommand{\inputpastL}        {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}      {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}      {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts}     { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \boldsymbol{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}      { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}      { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}       { \mathcal{F}}
\newcommand{\feedbackcausalstate}       { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}          { \mathcal{J}}
\newcommand{\JointCausalStateSet}       { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}       { {\Omega}}
\newcommand{\naturestate}       { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}       { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}       {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}                   { {\widehat{\Prob}_N}}
\newcommand{\STRegion}                  { {\mathrm K}}
\newcommand{\STRegionVariable}          { K}
\newcommand{\stregionvariable}          { k}
\newcommand{\GlobalPast}                { \overleftarrow{G}}
\newcommand{\globalpast}                { \overleftarrow{g}}
\newcommand{\GlobalFuture}              { \overrightarrow{G}}
\newcommand{\globalfuture}              { \overrightarrow{g}}
\newcommand{\GlobalState}               { \mathcal{G}}
\newcommand{\globalstate}               { \gamma}
\newcommand{\GlobalStateSet}            { {\mathbf \GlobalState}}
\newcommand{\LocalPast}                 { \overleftarrow{L}}
\newcommand{\localpast}                 { \overleftarrow{l}}
\newcommand{\AllLocalPasts}             { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}           { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}               { \overrightarrow{L}}
\newcommand{\localfuture}               { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}         { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}                { \mathcal{L}}
\newcommand{\localstate}                { \lambda}
\newcommand{\LocalStateSet}             { {\mathbf \LocalState}}
\newcommand{\PatchPast}                 { \overleftarrow{P}}
\newcommand{\patchpast}                 { \overleftarrow{p}}
\newcommand{\PatchPastRegion}           { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}               { \overrightarrow{P}}
\newcommand{\patchfuture}               { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}         { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}                { \mathcal{P}}
\newcommand{\patchstate}                { \pi}
\newcommand{\PatchStateSet}             { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}        {\vec{\LocalState}}
\newcommand{\localstatesinpatch}        {\vec{\localstate}}
\newcommand{\PointInstantX}             { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}                     { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}        {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]        { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]        { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]              { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]              { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}      { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess}     { {\Process}^{\forward} }
\newcommand{\PastProcess}       { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}      { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}             { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}             { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}      { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}        { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}              { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}             { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps}     { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}            {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}        { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}        { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\CausalState_{\lastindex{#1}{#2}}]}%
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}

\newcommand{\GI}{\ensuremath{\varphi}\xspace}
\newcommand{\OI}{\ensuremath{\zeta}\xspace}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{\ensuremath{k_{\PC}}\xspace}
\newcommand{\GOrder}{\ensuremath{k_{\GI}}\xspace}
\newcommand{\OOrder}{\ensuremath{k_{\OI}}\xspace}
\newcommand{\MOrder}{\ensuremath{R}\xspace}
\newcommand{\SOrder}{\ensuremath{k_{\SI}}\xspace}


%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}
\newcommand{\CSjointKL}[3][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState_{#2}\!#1\PastCausalState_{#3}}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState_{#2}#1\PastCausalState_{#3}}
   \fi
}


%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metric quantities of information generation, eg anatomy of a bit

\newcommand{\metric}[1] {\ensuremath{#1_\mu}\xspace}

\renewcommand{\hmu}{\metric{h}}
\newcommand{\rhomu}{\metric{\rho}}
\newcommand{\rmu}{\metric{r}}
\newcommand{\bmu}{\metric{b}}
\newcommand{\qmu}{\metric{q}}
\newcommand{\wmu}{\metric{w}}
\newcommand{\imu}{\metric{i}}
\newcommand{\sigmamu}{\metric{\sigma}}

\newcommand{\himc}{\ensuremath{h_{imc}}\xspace}
\newcommand{\pee}{\ensuremath{pee}\xspace} % parallel edge entropy

\newcommand{\ExE}[1] {\ensuremath{\EE_{#1}}\xspace}

\newcommand{\EER}{\ExE{R}}
\newcommand{\EEB}{\ExE{B}}
\newcommand{\EEQ}{\ExE{Q}}
\newcommand{\EEW}{\ExE{W}}
\newcommand{\EI}{\mathbf{I}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series, using the python-esque notation

\newcommand{\MS} [2] {\ensuremath{\MeasSymbol_{#1:#2}}\xspace}
\newcommand{\ms} [2] {\ensuremath{\meassymbol_{#1:#2}}\xspace}

\renewcommand{\Past}       {\MS{}{0}}
\newcommand{\Present}      {\ensuremath{\MeasSymbol_{0}}\xspace}
\renewcommand{\Future}     {\MS{0}{}}
\newcommand{\LPresent} [1] {\MS{0}{#1}}
\newcommand{\LFuture}  [1] {\MS{#1}{}}

\renewcommand{\past}       {\ms{}{0}}
\newcommand{\present}      {\ensuremath{\meassymbol_{0}}\xspace}
\renewcommand{\future}     {\ms{0}{}}
\newcommand{\lpresent} [1] {\ms{0}{#1}}
\newcommand{\lfuture}  [1] {\ms{#1}{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Causal states

\newcommand{\FCS}{\CausalState^\forward\xspace}
\newcommand{\RCS}{\CausalState^\reverse\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Others

\newcommand{\half}{\ensuremath{\nicefrac{1}{2}}}

\newcommand{\Language} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Lsync} {\Language_{\mathrm{sync}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathclap, in case someone doesn't have mathtools

% TUGboat, Volume 0 (2001), No. 0
% http://math.arizona.edu/~aprl/publications/mathclap/perlis_mathclap_24Jun2003.pdf
% For comparison, here are the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
%
% These are provided by mathtools
%
\ifcsname mathclap\endcsname
  \relax
\else
  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathllap{\mathpalette\mathllapinternal}
  \def\mathrlap{\mathpalette\mathrlapinternal}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathllapinternal#1#2{%
    \llap{$\mathsurround=0pt#1{#2}$}}
  \def\mathrlapinternal#1#2{%
    \rlap{$\mathsurround=0pt#1{#2}$}}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}}
\fi


==> infotheory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Information theory macros

\def \mid {~\middle|~}

% functions
\newcommand{\op} [3] [] {
  \ensuremath{
    \operatorname{#2_{#1}}
    \if\relax\detokenize{#3}\relax
    \else
      \left[ #3 \right]
    \fi
  }
  \xspace
}

% entropies
\renewcommand{\H}  [2] []       {\op[#1]{H}{#2}}
\newcommand{\ReE}  [2] [\alpha] {\H[#1]{#2}}
\newcommand{\TsE}  [2] [q]      {\op[#1]{S}{#2}}
\newcommand{\CRE}  [2] []       {\op[#1]{\mathcal{E}}{#2}}
\newcommand{\GCRE} [2] []       {\op[#1]{\mathcal{E^\prime}}{#2}}

% mutual informations
\newcommand{\I}  [2] [] {\op[#1]{I}{#2}}
\newcommand{\T}  [2] [] {\op[#1]{T}{#2}}
\newcommand{\B}  [2] [] {\op[#1]{B}{#2}}
\newcommand{\J}  [2] [] {\op[#1]{J}{#2}}
\newcommand{\II} [2] [] {\op[#1]{II}{#2}}

% common informations
\newcommand{\K} [2] [] {\op[#1]{K}{#2}}
\newcommand{\C} [2] [] {\op[#1]{C}{#2}}
\newcommand{\G} [2] [] {\op[#1]{G}{#2}}
\newcommand{\F} [2] [] {\op[#1]{F}{#2}}
\newcommand{\M} [2] [] {\op[#1]{M}{#2}}

% transfer entropies
\newcommand{\TE} [2] {\ensuremath{\operatorname{T}_{#1\rightarrow#2}}\xspace}
\newcommand{\CE} [3] {\ensuremath{\operatorname{\mathcal{C}}_{#1\rightarrow#2|#3}}\xspace}

% others
\renewcommand{\P}  [2] [] {\op[#1]{P}{#2}}
\newcommand{\X}    [2] [] {\op[#1]{X}{#2}}
\newcommand{\R}    [2] [] {\op[#1]{R}{#2}}
\newcommand{\D}    [2] [] {\op[#1]{D}{#2}}
\newcommand{\LMRP} [2] [] {\op[#1]{C_{\textrm{LMRP}}}{#2}}
\newcommand{\TSE}  [2] [] {\op[#1]{TSE}{#2}}

% divergences
\newcommand{\divergence} [3] {\ensuremath{\operatorname{#1}\left[#2~\middle|\middle|~#3\right]}\xspace}

\newcommand{\xH}  [2] {\divergence{xH}{#1}{#2}}
\newcommand{\DKL} [2] {\divergence{D_{KL}}{#1}{#2}}
\newcommand{\JSD} [2] {\divergence{D_{JS}}{#1}{#2}}

% operators on random variables
\newcommand{\meet}      {\curlywedge}
\newcommand{\join}      {\curlyvee}
\newcommand{\iless}     {\preceq}
\newcommand{\imore}     {\succeq}
\newcommand{\ieq}       {\cong}
\newcommand{\mss}       {\searrow}
\newcommand{\markov}    {\small{\mbox{$-\hspace{-1.3mm} \circ \hspace{-1.3mm}-$}}}

\newcommand{\ind}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}

\DeclareMathOperator*{\meetop}{\scalerel*{\meet}{\textstyle\sum}}
\DeclareMathOperator*{\joinop}{\scalerel*{\join}{\textstyle\sum}}

